Channel State Information Based Localization with Deep Learning

Localization is one of the most important problems in various fields such as robotics and wireless communications. For instance, Unmanned Aerial Vehicles (UAVs) require the information of the position precisely for an adequate control strategy. This problem is handled very efficiently with integrated GPS units for outdoor applications. However, indoor applications require special treatment due to the unavailability of GPS signals. Another aspect of mobile robots such as UAVs is that there is constant wireless communication between the mobile robot and a computational unit. This communication is mainly done for obtaining telemetry information or computation of control actions directly. The responsible integrated units for this transmission are commercial wireless communication chipsets. These units on the receiver side are responsible for getting rid of the diverse effects of the communication channel with various mathematical techniques. These techniques mainly require the Channel State Information (CSI) of the current channel to compensate the channel itself. After the compensation, the chipset has nothing to do with CSI. However, the locations of both the transmitter and receiver have a direct impact on CSI. Even though CSI contains such rich information about the environment, the accessibility of these data is blocked by the commercial wireless chipsets since they are manufactured to provide only the processed information data bits to the user. However, with the IEEE 802.11n standardization, certain chipsets provide access to CSI. Therefore, CSI data became processible and integrable to localization schemes. In this project, a test environment was constructed for the localization task. Two routers with proper chipsets were assigned as transmitter and receiver. They were operationalized for the CSI data collection. Lastly, these data were processed with various deep learning models.

==> Others/sembol.tex <==
\begin{tabular}{lrl}
{$\alpha$}              & : & Alpha  \\
{$\beta$}               & : & Beta \\
\end{tabular}

